Resolving Mutually Coherent Bright Point-Sources

We analyze the problem of resolving two point-sources in the case of mutually coherent sources with arbitrary quantum statistics, mutual phase, relative and absolute intensity. We use a sensitivity measure based on the method of moments and compare direct imaging with spatial mode demultiplexing, analytically proving the advantage of the latter. We show that the sensitivity of spatial mode demultiplexing saturates the quantum Fisher information, for all known cases, even for non-Gaussian states of the sources.

==> GoogleDriveLinks.tex <==
fig1.scheme.png
https://drive.google.com/uc?export=download&id=16rhTU04Vrypl0KIlwm3QYSswxXLo_V6j

fig1.scheme.pdf
https://drive.google.com/uc?export=download&id=1BxQk0EXRFPR1dFfyKIhpNF_Ps5j3eQ-x

plotDI1.pdf
https://drive.google.com/uc?export=download&id=187Q4pogNmZDgSZvIIY0vw-7g45ah3VUu

plotDI2.pdf
https://drive.google.com/uc?export=download&id=187_7lmkc0WaHGtOHakQa2nrWVtB825i4

legDI.pdf
https://drive.google.com/uc?export=download&id=18Cn8WT5YN52QzssM6ZD-wqFX6jIpHRne

plotHG.pdf
https://drive.google.com/uc?export=download&id=193e0-jJHAsPBm_VvzIldbxqjG9QJND5_

legHG.pdf
https://drive.google.com/uc?export=download&id=196H41WDIXKOGlK1W0lucl-A9YVZLt4Of

plotHGvsDI1.pdf
https://drive.google.com/uc?export=download&id=1AeU8YCgaKUC6fUKfFd4qS2tNYtztqWTi

plotHGvsDI2.pdf
https://drive.google.com/uc?export=download&id=1Av74kaG3j2TmPNgsWXrxvpbgbTSXdFIb

legHGvsDI.pdf
https://drive.google.com/uc?export=download&id=1AydZA_yGGFhbiwc7E_Jad8ggtUcA8T2z

plotMD1.pdf
https://drive.google.com/uc?export=download&id=1Co63sj5QXBd_sgRURzHvMK8l5_8zf0-i

plotMD2.pdf
https://drive.google.com/uc?export=download&id=1CjofToGWVfjNHHBaMxYCFRQQADn5PIwj

plotMD3.pdf
https://drive.google.com/uc?export=download&id=1Ck_izO4oHIt09xRIpIK2IWQX7fXxku9V

plotM1.pdf
https://drive.google.com/uc?export=download&id=1E4kqUxBTakjoZH-HH4EqQOEfMNOic-va 

plotM2.pdf
https://drive.google.com/uc?export=download&id=1E0F9okY4WbpCIOwP9Fuk3sxKRtcS0D8L 

plotM3.pdf
https://drive.google.com/uc?export=download&id=1DqR8bvc_T918V7ZdRK-TTlInYr8M9QKa 

plotM4DI.pdf
https://drive.google.com/uc?export=download&id=1FB_ecwNUQVAJvLC76c6oMRxY33uylzZp

legHGQFI.pdf
https://drive.google.com/uc?export=download&id=1K1LOTKiPDH3SFTVNjuP1bwNuOPd4Hmsn
